Bi-level Alignment for Cross-Domain Crowd Counting

Recently, crowd density estimation has received increasing attention. The main challenge for this task is to achieve high-quality manual annotations on a large amount of training data. To avoid reliance on such annotations, previous works apply unsupervised domain adaptation (UDA) techniques by transferring knowledge learned from easily accessible synthetic data to real-world datasets. However, current state-of-the-art methods either rely on external data for training an auxiliary task or apply an expensive coarse-to-fine estimation. In this work, we aim to develop a new adversarial learning based method, which is simple and efficient to apply. To reduce the domain gap between the synthetic and real data, we design a bi-level alignment framework (BLA) consisting of (1) task-driven data alignment and (2) fine-grained feature alignment. In contrast to previous domain augmentation methods, we introduce AutoML to search for an optimal transform on source, which well serves for the downstream task. On the other hand, we do fine-grained alignment for foreground and background separately to alleviate the alignment difficulty. We evaluate our approach on five real-world crowd counting benchmarks, where we outperform existing approaches by a large margin. Also, our approach is simple, easy to implement and efficient to apply. The code is publicly available at https://github.com/Yankeegsj/BLA.

==> CVPR2022 camera-ready/illustration/DR.tex <==
% \begin{table}[h]
% 	\centering
% 	\begin{tabular}{c|c|c}
% 		\toprule
% 		Method & MAE & MSE \\
% 		\hline
% 		\midrule
% 		Only Fine-grained Feature Alignment & 121.0 & 200.8 \\
% 		\midrule
% 		+ Standard Data Augmentation & 106.7 & 159.6 \\

% 		\midrule
% 		+ Our Transform Method  & 99.3 & 145.0 \\
% 		\hline
% 	\end{tabular}
% 	\caption{\newrevise{Efficiency of our transform method. }}
% 	\label{table:transform}
% \end{table}


\begin{table}[h]
	\centering
	\begin{tabular}{c|c|c}
		\toprule
		Method & MAE & MSE \\
		\hline
		\midrule
		Standard Data Augmentation & 106.7 & 159.6 \\

		\midrule
		Split and Transform & 99.3 & 145.0 \\
		\hline
	\end{tabular}
	\caption{\newrevise{Efficiency of our split and transform method. }}
	\label{table:transform}
\end{table}

==> CVPR2022 camera-ready/illustration/STOA.tex <==
% \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
% \begin{table*}[th]
% \small
% 	\renewcommand*{\arraystretch}{1.15}
% 	\centering
% 	\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
% 		\toprule
% 		\multirow{2}{*}{Method}&\multicolumn{2}{c|}{SHA}&\multicolumn{2}{c|}{SHB}&\multicolumn{2}{c|}{QNRF}
% 		&\multicolumn{2}{c|}{UCF-CC-50} &WorldExpo'10 \\
% 		\cline{2-10} 
% 		~ &MAE& MSE & MAE& MSE& MAE& MSE & MAE& MSE & Avg. MAE\\
% 		\hline
% 		\midrule
% 		NoAdpt \cite{cyclegan}& 160.0 &216.5& 22.8 & 30.6 & 275.5 & 458.5 & 487.2 & 689.0 & 42.8\\ \midrule
% 		Cycle-GAN \cite{cyclegan} & 143.3 & 204.3 & 25.4 & 39.7 & 257.3 & 400.6 & 404.6 & 548.2 & 26.3\\ \midrule
% 		SE Cycle-GAN \cite{GCC}& 123.4 & 193.4 & 19.9 & 28.3 & 230.4 &384.5 & 373.4 & 528.8 & 26.3\\ \midrule
% % 		SE Cycle-GAN(JT) \cite{cycleganjt} & 119.6 & 189.1 & 16.4 & 25.8 & 225.9 &385.7 & 370.2 & 512.0 & 24.4\\ \midrule
% 		SE Cycle-GAN(JT) \cite{cycleganjt} & 119.6 & 189.1 & 16.4 & 25.8 & 225.9 &385.7 & 370.2 & 512.0 & 24.4\\ \midrule
% 		FSC \cite{FSC}& 129.3 & 187.6 & 16.9 & 24.7 & 221.2 & 390.2 & - & - & -\\ \midrule
% 		FADA \cite{FADA}& - & - & 16.0 & 24.7 & - & - & - & - & 21.6\\  \midrule
% 		GP \cite{GP}& 121.0 & 181.0 & 12.8 & 19.2 & 210.0 &351.0 & 355.0 & 505.0 & 20.4\\ \hline \midrule
% 		% NoAdpt & 206.7 & 297.1 & 24.8 & 34.7 & 292.6 & 450.7 & - & - & 38.0\\ \midrule
% 		% DACC & 112.4 & 176.9 & 13.1 & 19.4 &211.7 & 357.9 & - & - &17.4\\ \midrule
		
% 		BLA (ours) & \textbf{99.3} & \textbf{145.0} & \textbf{11.9} & \textbf{18.9} & \textbf{198.9} &\textbf{316.1}& \textbf{346.8} & \textbf{480.0} & \textbf{17.9}\\ 
% % 		Searched transform $d$ &\multicolumn{2}{c|}{\textbf{[0.78,0.77,$\bm{12^{\circ}}$]} 
% % }&\multicolumn{2}{c|}{\textbf{[0.16,0.42,$\bm{3^{\circ}}$]}}&\multicolumn{2}{c|}{\textbf{[0.67, 0.41,$\bm{25^{\circ}}$]}}
% % 		&\multicolumn{2}{c|}{\textbf{[0.85,0.23,$\bm{4^{\circ}}$]}} &\textbf{[0.98,0.57,$\bm{17^{\circ}}$] }\\
% 		\hline
% 	\end{tabular}
% 	\caption{Comparison of our method with previous methods for synthetic-to-real adaptation. All methods employ VGG16 \cite{VGG} as backbone.}
% 	\label{table:STOA}
% \end{table*}

%
%\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
%\begin{table*}[th]
%	\small
%	\renewcommand*{\arraystretch}{1.15}
%	\centering
%	\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
%		\toprule
%		\multirow{2}{*}{Method}&\multirow{2}{*}{Backbone}&\multicolumn{2}{c|}{SHA}&\multicolumn{2}{c|}{SHB}&\multicolumn{2}{c|}{QNRF}
%		&\multicolumn{2}{c|}{UCF-CC-50} &WorldExpo'10 \\
%		\cline{3-11} 
%		~&~ &MAE& MSE & MAE& MSE& MAE& MSE & MAE& MSE & Avg. MAE\\
%		\hline
%		\midrule
%		NoAdpt \cite{cyclegan}&VGG& 160.0 &216.5& 22.8 & 30.6 & 275.5 & 458.5 & 487.2 & 689.0 & 42.8\\ \midrule
%		Cycle-GAN \cite{cyclegan}&VGG & 143.3 & 204.3 & 25.4 & 39.7 & 257.3 & 400.6 & 404.6 & 548.2 & 26.3\\ \midrule
%		SE Cycle-GAN \cite{GCC}&VGG& 123.4 & 193.4 & 19.9 & 28.3 & 230.4 &384.5 & 373.4 & 528.8 & 26.3\\ \midrule
%		% 		SE Cycle-GAN(JT) \cite{cycleganjt} & 119.6 & 189.1 & 16.4 & 25.8 & 225.9 &385.7 & 370.2 & 512.0 & 24.4\\ \midrule
%		SE Cycle-GAN(JT) \cite{cycleganjt}&VGG & 119.6 & 189.1 & 16.4 & 25.8 & 225.9 &385.7 & 370.2 & 512.0 & 24.4\\ \midrule
%		FSC \cite{FSC}&VGG& 129.3 & 187.6 & 16.9 & 24.7 & 221.2 & 390.2 & - & - & -\\ \midrule
%		FADA \cite{FADA}&VGG& - & - & 16.0 & 24.7 & - & - & - & - & 21.6\\  \midrule
%		GP \cite{GP}&VGG& 121.0 & 181.0 & 12.8 & 19.2 & 210.0 &351.0 & 355.0 & 505.0 & 20.4\\ \hline \midrule
%		% NoAdpt & 206.7 & 297.1 & 24.8 & 34.7 & 292.6 & 450.7 & - & - & 38.0\\ \midrule
%		% DACC & 112.4 & 176.9 & 13.1 & 19.4 &211.7 & 357.9 & - & - &17.4\\ \midrule
%		
%		BLA (ours) &VGG& \textbf{99.3} & \textbf{145.0} & \textbf{11.9} & \textbf{18.9} & \textbf{198.9} &\textbf{316.1}& \textbf{346.8} & \textbf{480.0} & \textbf{17.9}\\ 
%		% 		Searched transform $d$ &\multicolumn{2}{c|}{\textbf{[0.78,0.77,$\bm{12^{\circ}}$]} 
%		% }&\multicolumn{2}{c|}{\textbf{[0.16,0.42,$\bm{3^{\circ}}$]}}&\multicolumn{2}{c|}{\textbf{[0.67, 0.41,$\bm{25^{\circ}}$]}}
%		% 		&\multicolumn{2}{c|}{\textbf{[0.85,0.23,$\bm{4^{\circ}}$]}} &\textbf{[0.98,0.57,$\bm{17^{\circ}}$] }\\
%		\hline
%	\end{tabular}
%	\caption{Comparison of our method with previous methods for synthetic-to-real adaptation.}
%	\label{table:STOA}
%\end{table*}




\begin{table*}[h]
% \small
	\renewcommand*{\arraystretch}{1.15}
	\centering
	\begin{tabular}{cccccccccc}
		\toprule
		\multirow{2}{*}{Method}&\multicolumn{2}{c}{SHA}&\multicolumn{2}{c}{SHB}&\multicolumn{2}{c}{QNRF}
		&\multicolumn{2}{c}{UCF-CC-50} &WorldExpo'10 \\
		\cline{2-10} 
		~ &MAE& MSE & MAE& MSE& MAE& MSE & MAE& MSE & Avg. MAE\\
		\toprule
		NoAdpt \cite{cyclegan}& 160.0 &216.5& 22.8 & 30.6 & 275.5 & 458.5 & 487.2 & 689.0 & 42.8\\
		Cycle-GAN \cite{cyclegan} & 143.3 & 204.3 & 25.4 & 39.7 & 257.3 & 400.6 & 404.6 & 548.2 & 26.3\\ 
		SE Cycle-GAN \cite{GCC}& 123.4 & 193.4 & 19.9 & 28.3 & 230.4 &384.5 & 373.4 & 528.8 & 26.3\\ 
% 		SE Cycle-GAN(JT) \cite{cycleganjt} & 119.6 & 189.1 & 16.4 & 25.8 & 225.9 &385.7 & 370.2 & 512.0 & 24.4\\ \midrule
		SE Cycle-GAN(JT) \cite{cycleganjt} & 119.6 & 189.1 & 16.4 & 25.8 & 225.9 &385.7 & 370.2 & 512.0 & 24.4\\ 
		FSC \cite{FSC}& 129.3 & 187.6 & 16.9 & 24.7 & 221.2 & 390.2 & - & - & -\\ 
		FADA \cite{FADA}& - & - & 16.0 & 24.7 & - & - & - & - & 21.6\\ 
		GP \cite{GP}& 121.0 & 181.0 & 12.8 & 19.2 & 210.0 &351.0 & 355.0 & 505.0 & 20.4\\ 
% 		DACC [4]& 112.4 & 13.1  & 211.7 & \textbf{17.4}\\ \toprule
		
		% NoAdpt & 206.7 & 297.1 & 24.8 & 34.7 & 292.6 & 450.7 & - & - & 38.0\\ \midrule
		DACC \cite{gao2019domain}& 112.4 & 176.9 & 13.1 & 19.4 &211.7 & 357.9 & - & - &\textbf{17.4}\\ 
		\toprule
		BLA (ours) & \textbf{99.3} & \textbf{145.0} & \textbf{11.9} & \textbf{18.9} & \textbf{198.9} &\textbf{316.1}& \textbf{346.8} & \textbf{480.0} & 17.9\\ 
% 		Searched transform $d$ &\multicolumn{2}{c|}{\textbf{[0.78,0.77,$\bm{12^{\circ}}$]} 
% }&\multicolumn{2}{c|}{\textbf{[0.16,0.42,$\bm{3^{\circ}}$]}}&\multicolumn{2}{c|}{\textbf{[0.67, 0.41,$\bm{25^{\circ}}$]}}
% 		&\multicolumn{2}{c|}{\textbf{[0.85,0.23,$\bm{4^{\circ}}$]}} &\textbf{[0.98,0.57,$\bm{17^{\circ}}$] }\\
		\toprule
	\end{tabular}
	\caption{Comparison of our method with previous methods for synthetic-to-real adaptation. All methods employ VGG16 \cite{VGG} as backbone.}
	\label{table:STOA}
\end{table*}

==> CVPR2022 camera-ready/illustration/ablation.tex <==


% \begin{table}[h]
% 	\centering
% 	\small
% 	\begin{tabular}{c|c|c|c}
% 		\toprule
% 		\tabincell{c}{Task-Driven \\  Data Alignment} &\tabincell{c}{Fine-Grained \\  Feature Alignment}   & MAE &MSE \\
% 		\hline
% 		\midrule
% 		$\times$ & $\times$ & 134.7 & 210.9 \\
% 		\midrule
% 		\checkmark & $\times$ & 109.1 &153.8 \\
% 		\midrule
% 		$\times$ & \checkmark & 121.0&200.8 \\
% 		\midrule
% 		\checkmark & \checkmark& 99.3 & 145.0	\\
% 		\hline
% 	\end{tabular}
% 	\caption{Effects of two levels of alignment. 
% % 	\newrevise{For the 1st and 2nd rows, we replace fine-grained feature alignment with the most common global feature alignment. It is equivalent to the situation when the grid size $G$ of our local fine-grained feature alignment is set to the same size with the full image and the threshold of the foreground background $th$ is infinite.}
% % 	\shanshan{Let's reverse the 1st and 2nd columns, and the 121 and 109 rows. The idea is to put data alignment before feature alignment.}
% }
% 	\label{table:ablation}
% \end{table}

% \begin{table}[h]
% 	\centering
% 	\small
% 	\begin{tabular}{c|c|c|c}
% 		\toprule
% 		\tabincell{c}{Task-Driven \\  Data Alignment} &\tabincell{c}{Fine-Grained \\  Feature Alignment}   & MAE &MSE \\
% 		\hline
% 		\midrule
% 		$\times$ & $\times$ & 134.7 & 210.9 \\
% 		\midrule
% 		\checkmark & $\times$ & 109.1 &153.8 \\
% 		\midrule
% 		$\times$ & \checkmark & 121.0&200.8 \\
% 		\midrule
% 		\checkmark & \checkmark& 99.3 & 145.0	\\
% 		\hline
% 	\end{tabular}
% 	\caption{Effects of two levels of alignment. 
% % 	\newrevise{For the 1st and 2nd rows, we replace fine-grained feature alignment with the most common global feature alignment. It is equivalent to the situation when the grid size $G$ of our local fine-grained feature alignment is set to the same size with the full image and the threshold of the foreground background $th$ is infinite.}
% % 	\shanshan{Let's reverse the 1st and 2nd columns, and the 121 and 109 rows. The idea is to put data alignment before feature alignment.}
% }
% 	\label{table:ablation}
% \end{table}


\begin{table}[h]
	\centering
% 	\small
	\begin{tabular}{cccc}
		\toprule
		\tabincell{c}{Task-Driven \\  Data Alignment} &\tabincell{c}{Fine-Grained \\  Feature Alignment}   & MAE &MSE \\
		\toprule
		$\times$ & $\times$ & 134.7 & 210.9 \\
		\checkmark & $\times$ & 109.1 &153.8 \\
		$\times$ & \checkmark & 121.1&200.8 \\
		\checkmark & \checkmark& 99.3 & 145.0	\\
		\toprule
	\end{tabular}
	\caption{Effects of two levels of alignment. 
% 	\newrevise{For the 1st and 2nd rows, we replace fine-grained feature alignment with the most common global feature alignment. It is equivalent to the situation when the grid size $G$ of our local fine-grained feature alignment is set to the same size with the full image and the threshold of the foreground background $th$ is infinite.}
% 	\shanshan{Let's reverse the 1st and 2nd columns, and the 121 and 109 rows. The idea is to put data alignment before feature alignment.}
}
	\label{table:ablation}
\end{table}

==> CVPR2022 camera-ready/illustration/adain.tex <==
% \begin{figure}
% 	\begin{center}
% 		% \includegraphics[width=0.95\textwidth]{imgs/module.pdf}
% 		\includegraphics[width=0.5\textwidth]{figs/seed10086_all_point_del_three_points.png}
% 	\end{center}
% 	\caption{Target MAE and validation MAE}
% 	\label{adain}
% \end{figure}


\begin{figure}[h]
  \centering
  \includegraphics[scale=0.25]{figs/seed10086_del_5points.pdf}
  \hspace{1em}
  \includegraphics[scale=0.25]{figs/Target_MAE_del5points.pdf}
  \caption{Comparison of validation performance on the generated set (left) and real target set (right) across different transforms w.r.t. MAE. The similar trend verifies the effect of our validation feature generator. 
%   Concrete numbers are provided in the supplementary.
  }
\vspace{-10pt}
  \label{adain}
\end{figure}


==> CVPR2022 camera-ready/illustration/analysis.tex <==
% \begin{table}
%     % \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
% 	\centering
% 	\begin{tabular}{c|c|c|c|c}
% 		\toprule
% 		RGB2Gray & Scaling & \tabincell{c}{Perspective \\  transform}  &MAE &MSE \\
% 		\hline
% 		\midrule
% 		0. &1.0 &$0^{\circ}$ & 121.1 & 200.8 \\
% 		\midrule
% 		0.25 &1.0 &$0^{\circ}$ & 121.3 & 180.4 \\
% 		\midrule
% 		0.5 &1.0 &$0^{\circ}$ & \textbf{113.0} & \textbf{172.0} \\
% 		\midrule
% 		0.75 &1.0 &$0^{\circ}$ & 114.5 & 179.0 \\
% 		\midrule
% 		1.0 &1.0 &$0^{\circ}$ & 126.2 & 200.0 \\
% 		\midrule
% 		0.5 &0. &$0^{\circ}$ & 113.8 & 162.5 \\
% 		\midrule
% 		0.5 &0.25 &$0^{\circ}$ & 109.4 & 156.2 \\
% 		\midrule
% 		0.5 &0.5 &$0^{\circ}$ & \textbf{105.1} & \textbf{151.8} \\ 
% 		\midrule
% 		0.5 &0.75 &$0^{\circ}$ & 111.1 & 155.3 \\
% 		\midrule
% 		0.5 &0.5 &$11^{\circ}$ & 105.2 & 157.3 \\ 
% 		\midrule
% 		0.5 &0.5 &$22^{\circ}$ & 103.1 & 152.7 \\ 
% 		\midrule
% 		0.5 &0.5 &$33^{\circ}$ & 101.5 & \textbf{152.6} \\ 
% 		\midrule
% 		0.5 &0.5 &$45^{\circ}$ & \textbf{101.1} & 153.5 \\ 
% 		\hline
% 	\end{tabular}
% 	\caption{One by one grid search for parameters.}
% 	\label{table:gridsearch}
% \end{table}



\begin{table*}[h]
    % \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
	\centering
	\begin{tabular}{c|c|c|c|c|c}
		\toprule
		Index&p$_\text{G}$ & Scale factor & \tabincell{c}{Angle}  &MAE(generated set) &MAE (target set)\\
		\hline
		\midrule
		0&0.5 &0. &$0^{\circ}$  & 865.1& 113.8 \\
		\midrule
		1&0.5 &0.25 &$0^{\circ}$ &793.5& 109.4 \\
		\midrule
		2&0.5 &0.5 &$0^{\circ}$ & 800.4 & 105.1  \\ 
		\midrule
		3&0.5 &0.75 &$0^{\circ}$ & 775.5& 111.1 \\
		\midrule
		4&0.5 &0.5 &$11^{\circ}$ & 776.1& 105.2 \\ 
		\midrule
		5&0.5 &0.5 &$22^{\circ}$ & 797.9& 103.1\\ 
		\midrule
		6&0.5 &0.5 &$33^{\circ}$ & 789.2& 101.5 \\ 
		\midrule
		7&0.5 &0.5 &$45^{\circ}$ & 762.5& 101.1  \\ 
		\hline
	\end{tabular}
	\caption{The counting performance on our generated validation set and the real target training set.}
	\label{table:gridsearch}
\end{table*}

==> CVPR2022 camera-ready/illustration/backbone.tex <==
\begin{table}[h]
\small
\centering
	\begin{tabular}{c|c|c}
		\toprule
		Input &Layer&Output \\
		\hline
		\midrule
		\multicolumn{3}{c}{$\mathcal{F}$}\\
		\midrule
		3$\times$576$\times$768 & Conv:[k(3,3)-c64-s1-Relu] $\times$ 2 & 64$\times$576$\times$768\\
		\midrule
		64$\times$576$\times$768 & Maxpool:[k(2,2)-s2]  & 64$\times$288$\times$384\\
		\midrule
		64$\times$288$\times$384 & Conv:[k(3,3)-c128-s1-Relu]$\times$ 2  & 128$\times$288$\times$384\\
		\midrule
		128$\times$288$\times$384 & Maxpool:[k(2,2)-s2]  & 128$\times$144$\times$192\\
		\midrule
		128$\times$144$\times$192 & Conv:[k(3,3)-c256-s1-Relu]$\times$ 3  & 256$\times$144$\times$192\\
		\midrule
		256$\times$144$\times$192 & Maxpool:[k(2,2)-s2]  & 256$\times$72$\times$96\\
		\midrule
		256$\times$72$\times$96 & Conv:[k(3,3)-c512-s1-Relu] $\times$ 3 & 512$\times$72$\times$96\\
		\midrule
		\multicolumn{3}{c}{$\mathcal{E}$}\\
		\midrule
		512$\times$72$\times$96 & Conv:[k(3,3)-c128-s1-BN-Relu]  & 128$\times$72$\times$96\\
		\midrule
		128$\times$72$\times$96 & Deconv:[k(2,2)-c128-s2-BN-Relu]  & 128$\times$144$\times$192\\
		\midrule
		128$\times$144$\times$192 & Conv:[k(3,3)-c64-s1-BN-Relu]  & 64$\times$144$\times$192\\
		\midrule
		64$\times$144$\times$192 & Deconv:[k(2,2)-c64-s2-BN-Relu]  & 64$\times$288$\times$384\\
		\midrule
		64$\times$288$\times$384 & Conv:[k(3,3)-c32-s1-BN-Relu]  & 32$\times$288$\times$384\\
		\midrule
		32$\times$288$\times$384 & Deconv:[k(2,2)-c32-s2-BN-Relu]  & 32$\times$576$\times$768\\
		\midrule
		32$\times$576$\times$768 & Conv:[k(3,3)-c1-s1-Relu]  & 32$\times$576$\times$768\\
		\midrule
		\multicolumn{3}{c}{$\mathcal{D}$}\\
		\midrule
		512$\times$72$\times$96 & Conv:[k(3,3)-c512-s1-LeakyReLU]  & 512$\times$72$\times$96\\
		\midrule
		512$\times$72$\times$96 & Conv:[k(3,3)-c256-s1-LeakyReLU]  & 256$\times$72$\times$96\\
		\midrule
		256$\times$72$\times$96 & Conv:[k(3,3)-c2-s1]  & 2$\times$72$\times$96\\
		\midrule
		2$\times$72$\times$96 & Resize  & 2$\times(H/g_{h})\times (W/g_{w})$\\
		\midrule
		\multicolumn{3}{c}{$\mathcal{C}$}\\
		\midrule
		3 & FC:[c16-Relu]  & 16\\
		\midrule
		16 & FC:[c32-Relu]  & 32\\
		\midrule
		32 & FC:[c64-Relu]  & 64\\
		\midrule
		64 & FC:[c1-Relu]  & 1 ($\widetilde p_{k}$)\\
		\midrule
		64 & FC:[c32-Relu]  & 32\\
		\midrule
		32 & FC:[c16-Relu]  & 16\\
		\midrule
		16 & FC:[c3-Relu]  & 3 ($\widetilde d_{k}$)\\
		\hline
	\end{tabular}
	\caption{The network architecture of $\mathcal{F}, \mathcal{E}$, $\mathcal{D}$ and controller $\mathcal{C}$. }
	\label{table:backbone}
\end{table}



==> CVPR2022 camera-ready/illustration/da_dr_dl.tex <==
% \begin{figure}[t]
% 	\begin{center}
% 		% \includegraphics[width=0.95\textwidth]{imgs/module.pdf}
% 		\includegraphics[width=0.47\textwidth]{figs/DA_DR_dlv.pdf}
% 	\end{center}
% 	\caption{\shanshan{To be replaced with qualitative results of three different source augmentation methods, waiting for the style transfer model...}Comparison of three different ways for source domain augmentation. a. Domain randomization augments the source domain randomly without any priors from target; b. Style transfer translates images from source to a target-like domain based on target style priors, but the translation is hard to control and blind to the task objective; c. Our proposed task-driven data alignment augments the source domain based on both the target style priors and the task objective, which enables a more dynamic and robust model to the target domain.
% % 	style transfer translates images from source to target-like domain. Domain randomization generates new samples with random styles to enhance the generalization ability of the trained model. We combine the strengths of these two approaches and propose target-driven data-level alignment. We do source domain augmentation with target-style-related parameters. This enables the model to be both robust and adaptive to the target domain.
% 	}
% 	\label{DA_DR_dlv}
% \end{figure}

% \begin{figure*}[t]
% 	\begin{center}
% 		% \includegraphics[width=0.95\textwidth]{imgs/module.pdf}
% 		\includegraphics[width=0.95\textwidth]{figs/vision_dr_st_bla.pdf}
% 	\end{center}
% 	\caption{\shanshan{To be replaced with qualitative results of three different source augmentation methods, waiting for the style transfer model...}Comparison of three different ways for source domain augmentation. a. Domain randomization augments the source domain randomly without any priors from target; b. Style transfer translates images from source to a target-like domain based on target style priors, but the translation is hard to control and blind to the task objective; c. Our proposed task-driven data alignment augments the source domain based on both the target style priors and the task objective, which enables a more dynamic and robust model to the target domain.
% % 	style transfer translates images from source to target-like domain. Domain randomization generates new samples with random styles to enhance the generalization ability of the trained model. We combine the strengths of these two approaches and propose target-driven data-level alignment. We do source domain augmentation with target-style-related parameters. This enables the model to be both robust and adaptive to the target domain.
% 	}
% 	\label{DA_DR_dlv}
% \end{figure*}


% \begin{figure*}[t]
% 	\begin{center}
% 		% \includegraphics[width=0.95\textwidth]{imgs/module.pdf}
% 		\includegraphics[width=0.95\textwidth]{figs/vision_dr_st_bla.pdf}
% 	\end{center}
% 	\caption{\newrevise{Some qualitative results of three different source domain augmentation methods. For row 1, do data augmentation in RGB2Gray performs much better than style transfer. }
% % 	\shanshan{To be replaced with qualitative results of three different source augmentation methods, waiting for the style transfer model...}Comparison of three different ways for source domain augmentation. a. Domain randomization augments the source domain randomly without any priors from target; b. Style transfer translates images from source to a target-like domain based on target style priors, but the translation is hard to control and blind to the task objective; c. Our proposed task-driven data alignment augments the source domain based on both the target style priors and the task objective, which enables a more dynamic and robust model to the target domain.
% % 	style transfer translates images from source to target-like domain. Domain randomization generates new samples with random styles to enhance the generalization ability of the trained model. We combine the strengths of these two approaches and propose target-driven data-level alignment. We do source domain augmentation with target-style-related parameters. This enables the model to be both robust and adaptive to the target domain.
% 	}
% 	\label{DA_DR_dlv}
% \end{figure*}



% \begin{figure}[t]
% 	\begin{center}
% 		% \includegraphics[width=0.95\textwidth]{imgs/module.pdf}
% 		\includegraphics[width=0.47\textwidth]{figs/DA_DR_dlv.pdf}
% 	\end{center}
% 	\caption{\shanshan{To be replaced with qualitative results of three different source augmentation methods, waiting for the style transfer model...}Comparison of three different ways for source domain augmentation. a. Domain randomization augments the source domain randomly without any priors from target; b. Style transfer translates images from source to a target-like domain based on target style priors, but the translation is hard to control and blind to the task objective; c. Our proposed task-driven data alignment augments the source domain based on both the target style priors and the task objective, which enables a more dynamic and robust model to the target domain.
% % 	style transfer translates images from source to target-like domain. Domain randomization generates new samples with random styles to enhance the generalization ability of the trained model. We combine the strengths of these two approaches and propose target-driven data-level alignment. We do source domain augmentation with target-style-related parameters. This enables the model to be both robust and adaptive to the target domain.
% 	}
% 	\label{DA_DR_dlv}
% \end{figure}


% \begin{figure}

% \centering
% \begin{minipage}[t]{0.45\textwidth}
% \includegraphics[width=1\textwidth]{figs/style_transfer_subfig.pdf}
% \caption{Style Transfer.}
% \label{ForwardsmallF}
% \end{minipage}
% \begin{minipage}[t]{0.45\textwidth}
% \includegraphics[width=1\textwidth]{figs/task_driven_subfig.pdf}
% \end{minipage}
% \caption{aaaa} \label{fig:1}
% \end{figure}


\begin{figure} \centering
    \begin{subfigure}[a]{\linewidth}
    
    \begin{minipage}[t]{1\textwidth}
    \centering
\includegraphics[width=0.75\textwidth]{figs/style_transfer_subfig.pdf}
\caption{Style Transfer}
\end{minipage}
\begin{minipage}[t]{1\textwidth}
\centering
\includegraphics[width=0.9\textwidth]{figs/task_driven_subfig.pdf}
\caption{Domain Randomization and Task-Driven Data Alignment}
\end{minipage}
    \end{subfigure} %
\caption{Comparison of three different ways for source domain augmentation. (a). Style transfer translates images from source to a target-like domain based on target style priors, but the translation is usually limited to color changes, and blind to the task objective. (b). Domain randomization augments the source domain randomly in a more diverse manner (colors, scales, etc.) but without any priors from target; our proposed task-driven data alignment is more similar to domain randomization; but instead of random selection, we pick the most suitable augmentation based on the task objective, which enables a more dynamic and robust model to the target domain.}
\label{DA_DR_dlv}
\end{figure}




==> CVPR2022 camera-ready/illustration/datasets.tex <==


% \begin{table}[h]
% 	\centering
% 	\small
% 	\begin{tabular}{c|c|c|c}
% 		\toprule
% 		Dataset & Attribute  & \# Images   & Cnt (Mean $\pm$ Std)\\
% 		\hline
% 		\midrule
% 		GCC & Synthetic  & 15,211 &501$\pm$718\\
% 		\midrule
% 		SHA & Real-world &482&501$\pm$456\\
% 		\midrule
% 		SHB & Real-world &716 &123$\pm$94\\
% 		\midrule
% 		QNRF & Real-world& 1,535	& 815$\pm$1176\\
% 		\midrule
% 		UCF-CC-50 & Real-world &50 &1,279$\pm$950\\
% 		\midrule
% 		WorldExpo'10 & Real-world &3,980&50$\pm$41\\
% 		\hline
% 	\end{tabular}
	
% 	\caption{Statistics of five real-world datasets and one synthetic dataset GCC used for experiments.}
% 	\label{table:datasets}
% \end{table}
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\begin{table}[h]
	\centering
% 	\small
	\begin{tabular}{cccc}
% 		\toprule
% 		Dataset & Attribute  & \# Images   & Cnt (Mean $\pm$ Std)\\
% 		\toprule
% 		GCC & Synthetic  & 15,211 &501$\pm$718\\
% 		SHA & Real-world &482&501$\pm$456\\
% 		SHB & Real-world &716 &123$\pm$94\\
% 		QNRF & Real-world& 1,535	& 815$\pm$1176\\
% 		UCF-CC-50 & Real-world &50 &1,279$\pm$950\\
% 		WorldExpo'10 & Real-world &3,980&50$\pm$41\\
% 		\toprule
		\toprule
		Dataset & Attribute  & \# Images   & \tabincell{c}{Cnt \\(Mean $\pm$ Std)} \\
		\toprule
		GCC & Syn  & 15,211 &501$\pm$718\\
		SHA & Real &482&501$\pm$456\\
		SHB & Real &716 &123$\pm$94\\
		QNRF & Real& 1,535	& 815$\pm$1176\\
		UCF-CC-50 & Real &50 &1,279$\pm$950\\
		WorldExpo'10 & Real &3,980&50$\pm$41\\
		\toprule
	\end{tabular}
	
	\caption{Statistics of five real-world (Real) datasets and one synthetic (Syn) dataset GCC used for experiments.}
	\label{table:datasets}
\end{table}

==> CVPR2022 camera-ready/illustration/different_dataset.tex <==

% \begin{table}[th]
% \small
% 	\renewcommand*{\arraystretch}{1.15}
% 	\centering
% 	\begin{tabular}{c|c|c|c|c}
% 		\toprule
% 		\multirow{2}{*}{Dataset}&\multicolumn{2}{c|}{[0.78, 0.77, $12^{\circ}$]}&\multicolumn{2}{c}{[0.16, 0.42, $3^{\circ}$]}\\
% 		\cline{2-5} 
% 		~ &MAE& MSE & MAE& MSE\\
% 		\hline
% 		\midrule
% 		SHA& 99.3 &145.0& 104.3 & 153.7 \\ \midrule
% 		SHB& 14.7 & 26.4 & 11.9 & 18.9 \\ 
% % 		Searched transform $d$ &\multicolumn{2}{c|}{\textbf{[0.78,0.77,$\bm{12^{\circ}}$]} 
% % }&\multicolumn{2}{c|}{\textbf{[0.16,0.42,$\bm{3^{\circ}}$]}}&\multicolumn{2}{c|}{\textbf{[0.67, 0.41,$\bm{25^{\circ}}$]}}
% % 		&\multicolumn{2}{c|}{\textbf{[0.85,0.23,$\bm{4^{\circ}}$]}} &\textbf{[0.98,0.57,$\bm{17^{\circ}}$] }\\
% 		\hline
% 	\end{tabular}
% 	\caption{Different datasets require different transformation. Therefore, it is necessary to do task-driven search.}
% 	\label{table:different_dataset}
% \end{table}

% \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
% \begin{table}[th]
% \small
% 	\renewcommand*{\arraystretch}{1.15}
% 	\centering
% 	\begin{tabular}{c|c|c|c|c}
% 		\toprule
% 		\multirow{2}{*}{Dataset}&\multicolumn{2}{c|}{Searched $d$ for SHA}&\multicolumn{2}{c}{Searched $d$ for SHB}\\
% 		~&\multicolumn{2}{c|}{[0.78, 0.77, $12^{\circ}$]}&\multicolumn{2}{c}{[0.16, 0.42, $3^{\circ}$]}\\
% 		\cline{2-5} 
% 		~ &MAE& MSE & MAE& MSE\\
% 		\hline
% 		\midrule
% 		SHA& \textbf{99.3} &\textbf{145.0}& 104.3 & 153.7 \\ \midrule
% 		SHB& 14.7 & 26.4 & \textbf{11.9} & \textbf{18.9} \\ 
% % 		Searched transform $d$ &\multicolumn{2}{c|}{\textbf{[0.78,0.77,$\bm{12^{\circ}}$]} 
% % }&\multicolumn{2}{c|}{\textbf{[0.16,0.42,$\bm{3^{\circ}}$]}}&\multicolumn{2}{c|}{\textbf{[0.67, 0.41,$\bm{25^{\circ}}$]}}
% % 		&\multicolumn{2}{c|}{\textbf{[0.85,0.23,$\bm{4^{\circ}}$]}} &\textbf{[0.98,0.57,$\bm{17^{\circ}}$] }\\
% 		\hline
% 	\end{tabular}
% 	\caption{Different datasets require different transformations for optimal results.}
% 	\label{table:different_dataset}
% \end{table}



\begin{table}[h]
% \small
	\renewcommand*{\arraystretch}{1.15}
	\centering
	\begin{tabular}{ccccc}
		\toprule
		\multirow{2}{*}{Dataset}&\multicolumn{2}{c}{Searched $d$ for SHA}&\multicolumn{2}{c}{Searched $d$ for SHB}\\
		~&\multicolumn{2}{c}{[0.78, 0.77, $12^{\circ}$]}&\multicolumn{2}{c}{[0.16, 0.42, $3^{\circ}$]}\\
		\cline{2-5} 
		~ &MAE& MSE & MAE& MSE\\
		\toprule
		SHA& \textbf{99.3} &\textbf{145.0}& 104.3 & 153.7 \\ 
		SHB& 14.7 & 26.4 & \textbf{11.9} & \textbf{18.9} \\ 
% 		Searched transform $d$ &\multicolumn{2}{c|}{\textbf{[0.78,0.77,$\bm{12^{\circ}}$]} 
% }&\multicolumn{2}{c|}{\textbf{[0.16,0.42,$\bm{3^{\circ}}$]}}&\multicolumn{2}{c|}{\textbf{[0.67, 0.41,$\bm{25^{\circ}}$]}}
% 		&\multicolumn{2}{c|}{\textbf{[0.85,0.23,$\bm{4^{\circ}}$]}} &\textbf{[0.98,0.57,$\bm{17^{\circ}}$] }\\
		\toprule
	\end{tabular}
	\caption{Different datasets require different transformations for optimal results.}
	\vspace{-10pt}
	\label{table:different_dataset}
\end{table}

==> CVPR2022 camera-ready/illustration/drstdla.tex <==
% \begin{table}[h]
% 	\centering
% 	\begin{tabular}{c|c|c}
% 		\toprule
% 		Method & MAE & MSE \\
% 		\hline
% 		\midrule
% 		Style Transfer  & 119.4& 194.6 \\ \midrule
% % 		Domain Randomization  & 110.0$\pm$2.4 & 164.2$\pm$8.9 \\ 
% 		Domain Randomization  & 110.0 & 164.2 \\ 
% 		\hline \midrule
% 		Task-Driven Data Alignment  & \textbf{99.3} & \textbf{145.0} \\
% 		\hline
% 	\end{tabular}
% 	\caption{Effect of Task-Driven Data Alignment.}
% 	\label{table:drstdla}
% \end{table}


\begin{table}[h]
	\centering
	\begin{tabular}{ccc}
		\toprule
		Method & MAE & MSE \\
		\toprule
		Style Transfer  & 119.4& 194.6 \\ 
% 		Domain Randomization  & 110.0$\pm$2.4 & 164.2$\pm$8.9 \\ 
		Domain Randomization  & 110.0 & 164.2 \\ 

		Task-Driven Data Alignment  & \textbf{99.3} & \textbf{145.0} \\
		\toprule
	\end{tabular}
	\caption{Effect of Task-Driven Data Alignment.}
	\label{table:drstdla}
\end{table}

==> CVPR2022 camera-ready/illustration/grid.tex <==
% \begin{table}[h]
% \small
% 	\centering
% 	\begin{tabular}{c|c|c}
% 		\toprule
% 		Grid size $G$ & MAE & MSE \\
% 		\hline
% 		\midrule
% 		(2,2) & 138.1 & 222.9 \\
% 		\midrule
% 		(4,4) & 130.5 & 205.4 \\
% 		\midrule
% 		(8,8) & 129.0 & 206.3 \\
% 		\midrule
% 		(16,16) & 121.1 & 200.8 \\
% 		\midrule
% 		(32,32) & 141.4 & 223.6 \\
% 		\hline
% 	\end{tabular}
% 	\caption{Impact of local grid size $G$ in fine-grained feature alignment.}
% 	\label{table:grid}
% \end{table}

\begin{table}[h]
% \small
	\centering
	\begin{tabular}{ccc}
		\toprule
		Grid size $G$ & MAE & MSE \\
		\toprule
		(2,2) & 138.1 & 222.9 \\
		(4,4) & 130.5 & 205.4 \\
		(8,8) & 129.0 & 206.3 \\
		(16,16) & 121.1 & 200.8 \\
		(32,32) & 141.4 & 223.6 \\
		\toprule
	\end{tabular}
	\caption{Impact of local grid size $G$ used in fine-grained feature alignment.
% 	\shanshan{highlight the best numbers in bold}
}
	\label{table:grid}
\end{table}

% \begin{table}[h]
% \small
% 	\centering
% 	\begin{tabular}{c|c|c|c}
% 		\toprule
% 		Grid size $G$ &(2,2)&(4,4)&(8,8) \\
% 		\hline
% 		\midrule
% 		MAE & 138.1  & 130.5& 129.0\\
% 		\midrule
% 		MSE& 222.9& 205.4& 206.3\\
% 		\midrule
% 		Grid size $G$ &(16,16)&(32,32)&(64,64)\\
% 		\hline
% 		\midrule
% 		MAE & 121.1& 141.4& 127.1\\
% 		\midrule
% 		MSE& 200.8& 223.6& 211.3\\
% 		\hline
% 	\end{tabular}
% 	\caption{Effect of different local grid size $G$.}
% 	\label{table:grid}
% \end{table}

==> CVPR2022 camera-ready/illustration/grid_search_fig.tex <==
% \begin{figure*}
% \begin{center}

% \begin{minipage}[t]{0.3\linewidth} 
% 	\centering 
% 	\includegraphics[width=1\textwidth]{figs/RGB2Gray.pdf}
% 	\label{figure:grid search gray}
% \end{minipage}
% \hspace{1em}
%   \begin{minipage}[t]{0.3\linewidth} 
%   \centering 
%   \includegraphics[width=1\textwidth]{figs/Scaling.pdf}
%   \label{figure:grid search scale}
%   \end{minipage}
%  \hspace{1em}
%   \begin{minipage}[t]{0.3\linewidth} 
%   \centering 
%   \includegraphics[width=1\textwidth]{figs/PT.pdf}
%   \label{figure:grid search pt}
%   \end{minipage} 
% \end{center}
% \caption{From left to right we search for the three parameters in order. In the left figure, we search for RGB2Gray radio, we find the best radio is 0.5. When searching for the following parameters, we fixed the ratio at 0.5. }
% \label{model}
% \end{figure*}


\begin{figure*}[h]
  \centering
  \includegraphics[scale=0.32]{figs/RGB2Gray.pdf}
  \hspace{1em}
  \includegraphics[scale=0.32]{figs/Scaling.pdf}
  \hspace{1em}
  \includegraphics[scale=0.32]{figs/PT.pdf}
  \caption{\newrevise{From left to right we search for the three parameters in order. $P_G$, scale factor and angle are set to 0., 1.0 and $0^\circ$ by default. In the left figure, we search for $P_G$, and keep scale factor and angle as default, we find the best radio is 0.5. When searching for the following parameters, we fixed the ratio at 0.5. In following search, the parameters searched are fixed as found, and those not searched are kept as default.}
  }
  \label{fig:grid search}
\end{figure*}


==> CVPR2022 camera-ready/illustration/method.tex <==
\begin{figure*}
	\begin{center}
		% \includegraphics[width=0.95\textwidth]{imgs/module.pdf}
		\includegraphics[width=0.91\textwidth]{figs/RDS.pdf}
	\end{center}
	\caption{Overview of our proposed bi-level alignment framework (BLA), which mainly consists of four components: feature extractor $(\mathcal{F})$, density estimator $(\mathcal{E})$, task-driven data alignment and local fine-grained discriminator $(\mathcal{D})$. At training time, the source dataset $S$ is transformed to $S^+$ with the optimal transform searched via task-driven data alignment (Alg. \ref{data-level alignment}), during which the validation feature generator provides target-like features for candidate transform validation.
	Then the entire network is optimized based on $S^+$ and $T$ using the training objective in Eq. \ref{objective}.
	\textbf{At test time, we simply feed a target image $x_T^i$ to $\mathcal{F}$ and $\mathcal{E}$ to obtain the predicted density map $\widetilde y_T$}. 
% 	Please note that during the search process, we generate target-like image feature for candidate transform validation. 
% 	Then, we  retrain the network with the transformed $S^+$ obtained by searched transform.
	}
	\label{method}
\end{figure*}

==> CVPR2022 camera-ready/illustration/search_process.tex <==
%AAAI2022 sample
%\begin{algorithm}[tb]
%	\caption{Example algorithm}
%	\label{alg:algorithm}
%	\textbf{Input}: Your algorithm's input\\
%	\textbf{Parameter}: Optional list of parameters\\
%	\textbf{Output}: Your algorithm's output
%	\begin{algorithmic}[1] %[1] enables line numbers
%		\STATE Let $t=0$.
%		\WHILE{condition}
%		\STATE Do some action.
%		\IF {conditional}
%		\STATE Perform task A.
%		\ELSE
%		\STATE Perform task B.
%		\ENDIF
%		\ENDWHILE
%		\STATE \textbf{return} solution
%	\end{algorithmic}
%\end{algorithm}


%\begin{algorithm}[h]  
%	
%	\caption{Pseudo code of data-level alignment} 
%	\label{data-level alignment}
%	\begin{algorithmic}[l] 
%		\STATE Define number of search epochs $N_{epoch}$;
%		\STATE Define set of evaluation epochs $N_{eval}$;
%		\STATE Define gradient based controller $C$;
%		\STATE Define number of iterations in one epoch $N_{iter}$;
%		\STATE Initialize candidate architectures $A=\{A_{RGB}, A_{Pose}\}$;
%		\STATE Initialize the pre-defined fusion net $Net_{F}$ as Table~\ref{simple fusion net};
%		\FOR{$epoch \in [1,N_{epoch}]$}
%		\FOR{$iter \in [1,N_{iter}]$}
%		\STATE $a\gets$ random pick($A$)
%		\STATE $\{a_{RGB},a_{Pose}\} \gets$ $a$
%		\STATE train($\{a_{RGB}+a_{Pose}\}+Net_{F}$)
%		\ENDFOR
%		\IF{$epoch \in N_{eval}$}
%		\STATE $reward$ $\gets$ eval($A$);\COMMENT Acc in validation set;
%		\STATE train($C$);
%		\STATE generate $A_1$ by $C$;
%		\STATE reserve the top K architectures in $A$ as $A_2$;
%		\STATE randomly generate some architectures $A_3$;
%		\STATE update($A$)\COMMENT Combine $A_1$, $A_2$ and $A_3$;
%		\ENDIF
%		\ENDFOR
%		\STATE $top1$ $\gets$ pick($A$, $reward$);
%		\STATE $\{B_{RGB},B_{Pose}\} \gets$ $top1$;
%		\STATE $Net_{TS}=\{B_{RGB},B_{Pose}\}$
%		\STATE \textbf{Return} $Net_{TS}$
%		%       \textcolor{red}{This algorithm should return $Net_{TS}$ and end here.}
%		%       \STATE initialize $Net_{TS}$ and $Net_F$;
%		%       \STATE $Net_{TS}$ + $Net_F$ $\gets$train($Net_{TS}+Net_{F}$)\Comment From scratch;
%		%       \STATE \textbf{Return} $Net_{TS}$ + $Net_F$
%		
%	\end{algorithmic}
%\end{algorithm}  

% \begin{algorithm}[tb]  
\begin{algorithm}[!tb]  
	\caption{Pseudo code of one-round search procedure of data-level alignment} 
	\label{data-level alignment}
	\textbf{Input}: Source and target domain training set $S$, $T$; the pre-trained  source only network $\mathcal{\widehat{G}}=\{\widehat{\theta}_{\mathcal{F} },\widehat{\theta}_{\mathcal{E}}\}$; the candidate transform set  $\mathbb{D}$ and the controller $\mathcal{C}$ \par
	\begin{algorithmic}[1]
		\FOR{$d_k \in \mathbb{D}$}
		\STATE initialize $\mathcal{G}=\{\theta_{\mathcal{F}},\theta_{\mathcal{E}},\theta_{\mathcal{D}}\} $ with $\mathcal{\widehat{G}}$
		\STATE $S^+_k=$ transform ($S$,$d_k$)\COMMENT{\textsl{As Fig. \ref{split}}}
		\STATE $\mathcal{G}=$  train ($\mathcal{G},S^+_k,T$)
		\STATE $p_k=$ validate ($\mathcal{G},S,T$)
		\COMMENT{\textsl{Val performance as reward}}
		\ENDFOR
		\STATE $\mathbb{P}=\{p_1,p_2...\}$
		\STATE $\mathcal{C}=$ train controller($\mathcal{C},\mathbb{D},\mathbb{P}$) 
		\COMMENT{\textsl{As Eq. \ref{equation:controller}}}
		\STATE $\mathbb{D}=$ update ($\mathcal{C},\mathbb{D}$)
		\COMMENT{\textsl{Same with NAO \cite{NAO}}}
% 		\STATE $\mathbb{D}=$ update ($\mathbb{D'},\mathbb{D}$)
		\STATE \textbf{return} $\mathbb{D},\mathbb{P}$
	\end{algorithmic}
\end{algorithm} 

==> CVPR2022 camera-ready/illustration/search_space.tex <==



% \begin{table}[h]
% \small
% \renewcommand*{\arraystretch}{1.2}
% 	\centering
% 	\begin{tabular}{c|c|c}
% 		\toprule
% 		\multirow{2}{*}{Transform unit}  &\multicolumn{2}{c}{Parameters}\\ \cline{2-3} 
% 		 ~ &Split ratio &  Attribute\\
% 		\hline
% 		\midrule
% 		RGB2Gray & p$_\text{G}$* &- \\
% 		\midrule
% 		Scaling & p$_\text{S}$& Scale factor*  \\
% 		\midrule
% 		Perspective transform & p$_\text{PT}$& Angle* \\
% 		\hline
% 	\end{tabular}
% % 	\caption{Each transform consists of three different units. A full transform set is generated by iterating each parameter within its search space.}
% 	\caption{Each transform consists of three different units, each represented by two parameters: one for split ratio and another for attribute. * marks those parameters we search while others are fixed. A full transform set is generated by iterating each parameter.
% % 	For all our experiments, we search p$_\text{S}$, Scale factor and Angle, and both p$_\text{S}$ and p$_\text{PT}$ are set to 0.5.
% 	}
% 	\label{table:search_space}
% \end{table}

\begin{table}[h]
\small
\renewcommand*{\arraystretch}{1.2}
	\centering
	\begin{tabular}{ccc}
		\toprule
		\multirow{2}{*}{Transform unit}  &\multicolumn{2}{c}{Parameters}\\ \cline{2-3} 
		 ~ &Split ratio &  Attribute\\
		\toprule
		RGB2Gray & p$_\text{G}$* &- \\
		Scaling & p$_\text{S}$& Scale factor*  \\
		Perspective transform & p$_\text{PT}$& Angle* \\
		\toprule
	\end{tabular}
% 	\caption{Each transform consists of three different units. A full transform set is generated by iterating each parameter within its search space.}
	\caption{Each transform consists of three different units, each represented by two parameters: one for split ratio and another for attribute. * marks those parameters we search while others are fixed. A full transform set is generated by iterating each parameter.
% 	For all our experiments, we search p$_\text{S}$, Scale factor and Angle, and both p$_\text{S}$ and p$_\text{PT}$ are set to 0.5.
	}
	\label{table:search_space}
\end{table}




==> CVPR2022 camera-ready/illustration/searched_d.tex <==
% \begin{table}[h]
% \small
% 	\renewcommand*{\arraystretch}{1.1}
% 	\centering
% 	\begin{tabular}{c|c|c|c}
% 		\toprule
% 		\multirow{2}{*}{Dataset}&\multicolumn{3}{c}{Searched transform $d$} \\
% 		\cline{2-4} 
% 		~ &p$_\text{G}$& Scale factor & Angle\\
% 		\hline
% 		\midrule
% 		SHA&0.78&0.77&$12^{\circ}$\\
% 		\midrule
% 		SHB&0.16&0.42&$3^{\circ}$\\
% 		\midrule
% 		QNRF&0.67&0.41&$25^{\circ}$\\
% 		\midrule
% 		UCF-CC-50&0.85&0.23&$4^{\circ}$\\
% 		\midrule
% 		WorldExpo'10&0.98&0.57&$17^{\circ}$\\
% 		\hline
% 	\end{tabular}
% 	\caption{Searched transforms vary across different target datasets.}
% 	\label{table:searched_d}
% \end{table}

\begin{table}[h]
% \small
	\renewcommand*{\arraystretch}{1.1}
	\centering
	\begin{tabular}{cccc}
		\toprule
		\multirow{2}{*}{Dataset}&\multicolumn{3}{c}{Searched transform $d$} \\
		\cline{2-4} 
		~ &p$_\text{G}$& Scale factor & Angle\\
		\toprule
		SHA&0.78&0.77&$12^{\circ}$\\
		SHB&0.16&0.42&$3^{\circ}$\\
		QNRF&0.67&0.41&$25^{\circ}$\\
		UCF-CC-50&0.85&0.23&$4^{\circ}$\\
		WorldExpo'10&0.98&0.57&$17^{\circ}$\\
		\toprule
	\end{tabular}
	\caption{Searched transforms vary across different target datasets.}
	\label{table:searched_d}
	\vspace{-10pt}
\end{table}
% \vspace{-10pt}

==> CVPR2022 camera-ready/illustration/small_fig.tex <==
\begin{figure}[t]
	\begin{center}
		% \includegraphics[width=0.95\textwidth]{imgs/module.pdf}
		\includegraphics[width=0.45\textwidth]{figs/small_fig.pdf}
	\end{center}
	\caption{High intraclass diversity samples. Although
	instances belonging to the same class vary greatly  in color, shape and scale, we are required to count them without omission.
% 	\shanshan{The flow is unclear: what is input, loss; maybe we show the baseline and addons from us;}\comment{in progress}
	}
	\label{fig:small_fig}
\end{figure}

==> CVPR2022 camera-ready/illustration/split.tex <==
% \begin{figure*}
% 	\begin{center}
% 		% \includegraphics[width=0.95\textwidth]{imgs/module.pdf}
% 		\includegraphics[width=0.9\textwidth]{figs/split.pdf}
% 	\end{center}
% 	\caption{This is an illustration of how do we transform the source domain $S$ to a new mixed source dataset $S^+$. In terms of implementation, we split and transform (SAT) the original data to $S^+$. There are three transformations, so, there are 8 possibilities for each image. Different from data augmentation, each image has only one form during training. For instance, given $d=[RGB2Gray=0.75,Scaling=0.6,Perspective transform=10^{\circ}]$, for three transformations, we provide the probability of applying the transformation, which are $P(RGB2Gray)=0.75, P(Scaling)=0.5, P(Perspective transform)=0.5$ respectively. After transformation, we obtain $S^+$ which consists of 8 mixed transformation subset.}
% 	\label{split}
% \end{figure*}

\begin{figure}
	\begin{center}
		% \includegraphics[width=0.95\textwidth]{imgs/module.pdf}
		\includegraphics[width=0.46\textwidth]{figs/split.pdf}
	\end{center}
	\caption{We split the whole source set into several subsets via a transform tree according to p$_\text{G}$, p$_\text{S}$ and p$_\text{PT}$.
 ``\textbf{Y:} p$_\text{G}$'' refers to performing the transformation G with a ratio of p$_\text{G}$; ``\textbf{N:} 1 - p$_\text{G}$'' means that no transformation is performed with a ratio of 1 - p$_\text{G}$.
% 	Given $d_k$, p$_\text{G}$ equals to the first parameter of $d_k$; both p$_\text{S}$ and p$_\text{PT}$ are set to 0.5.
	Finally, we obtain the corresponding subsets as shown at the bottom row, which constitute $S^+$.
% 	\shanshan{currently, we use S for both source and scaling, which might be confusing for readers; try to use other letters or words for three units, e.g. 'Color','Scale', 'PT', or 'U1','U2','U3'. }
	}
	\label{split}
\end{figure}


==> CVPR2022 camera-ready/illustration/srvsst.tex <==
\begin{table}[h]
	\centering
	\begin{tabular}{c|c|c}
		\toprule
		Method & MAE & MSE \\
		\hline
		\midrule
		Cycle-GAN \cite{cyclegan} & 143.3 & 204.3 \\ \midrule
		SE Cycle-GAN \cite{GCC}& 123.4 & 193.4 \\ \midrule
% 		SE Cycle-GAN(JT) \cite{cycleganjt} & 119.6 & 189.1 & 16.4 & 25.8 & 225.9 &385.7 & 370.2 & 512.0 & 24.4\\ \midrule
		SE Cycle-GAN(JT) \cite{cycleganjt} & 119.6 & 189.1 \\  \hline \midrule
		Style Randomization  & 111.6 & 177.5 \\
		\hline
	\end{tabular}
	\caption{\revise{Style Randomization VS Style Transfer.transform(0.5,0.5,22)}}
	\label{table:srvsst}
\end{table}

==> CVPR2022 camera-ready/illustration/vision_results.tex <==
\begin{figure*}[t]
	\begin{center}
		% \includegraphics[width=0.95\textwidth]{imgs/module.pdf}
		\includegraphics[width=0.93\textwidth]{figs/vision_results.pdf}
	\end{center}
	   \vspace{-15pt}
	\caption{Qualitative adaptation results of images with different levels of density on SHA. 
% 	Please note that during the search process, we generate target-like image feature for candidate transform validation. 
% 	Then, we  retrain the network with the transformed $S^+$ obtained by searched transform.
	}
	\vspace{-10pt}
	\label{vision_results}
\end{figure*}

==> illustration/DR.tex <==
% \begin{table}[h]
% 	\centering
% 	\begin{tabular}{c|c|c}
% 		\toprule
% 		Method & MAE & MSE \\
% 		\hline
% 		\midrule
% 		Only Fine-grained Feature Alignment & 121.0 & 200.8 \\
% 		\midrule
% 		+ Standard Data Augmentation & 106.7 & 159.6 \\

% 		\midrule
% 		+ Our Transform Method  & 99.3 & 145.0 \\
% 		\hline
% 	\end{tabular}
% 	\caption{\newrevise{Efficiency of our transform method. }}
% 	\label{table:transform}
% \end{table}


\begin{table}[h]
	\centering
	\begin{tabular}{c|c|c}
		\toprule
		Method & MAE & MSE \\
		\hline
		\midrule
		Standard Data Augmentation & 106.7 & 159.6 \\

		\midrule
		Split and Transform & 99.3 & 145.0 \\
		\hline
	\end{tabular}
	\caption{\newrevise{Efficiency of our split and transform method. }}
	\label{table:transform}
\end{table}

==> illustration/analysis.tex <==
% \begin{table}
%     % \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
% 	\centering
% 	\begin{tabular}{c|c|c|c|c}
% 		\toprule
% 		RGB2Gray & Scaling & \tabincell{c}{Perspective \\  transform}  &MAE &MSE \\
% 		\hline
% 		\midrule
% 		0. &1.0 &$0^{\circ}$ & 121.1 & 200.8 \\
% 		\midrule
% 		0.25 &1.0 &$0^{\circ}$ & 121.3 & 180.4 \\
% 		\midrule
% 		0.5 &1.0 &$0^{\circ}$ & \textbf{113.0} & \textbf{172.0} \\
% 		\midrule
% 		0.75 &1.0 &$0^{\circ}$ & 114.5 & 179.0 \\
% 		\midrule
% 		1.0 &1.0 &$0^{\circ}$ & 126.2 & 200.0 \\
% 		\midrule
% 		0.5 &0. &$0^{\circ}$ & 113.8 & 162.5 \\
% 		\midrule
% 		0.5 &0.25 &$0^{\circ}$ & 109.4 & 156.2 \\
% 		\midrule
% 		0.5 &0.5 &$0^{\circ}$ & \textbf{105.1} & \textbf{151.8} \\ 
% 		\midrule
% 		0.5 &0.75 &$0^{\circ}$ & 111.1 & 155.3 \\
% 		\midrule
% 		0.5 &0.5 &$11^{\circ}$ & 105.2 & 157.3 \\ 
% 		\midrule
% 		0.5 &0.5 &$22^{\circ}$ & 103.1 & 152.7 \\ 
% 		\midrule
% 		0.5 &0.5 &$33^{\circ}$ & 101.5 & \textbf{152.6} \\ 
% 		\midrule
% 		0.5 &0.5 &$45^{\circ}$ & \textbf{101.1} & 153.5 \\ 
% 		\hline
% 	\end{tabular}
% 	\caption{One by one grid search for parameters.}
% 	\label{table:gridsearch}
% \end{table}



\begin{table*}[h]
    % \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
	\centering
	\begin{tabular}{c|c|c|c|c|c}
		\toprule
		Index&p$_\text{G}$ & Scale factor & \tabincell{c}{Angle}  &MAE(generated set) &MAE (target set)\\
		\hline
		\midrule
		0&0.5 &0. &$0^{\circ}$  & 865.1& 113.8 \\
		\midrule
		1&0.5 &0.25 &$0^{\circ}$ &793.5& 109.4 \\
		\midrule
		2&0.5 &0.5 &$0^{\circ}$ & 800.4 & 105.1  \\ 
		\midrule
		3&0.5 &0.75 &$0^{\circ}$ & 775.5& 111.1 \\
		\midrule
		4&0.5 &0.5 &$11^{\circ}$ & 776.1& 105.2 \\ 
		\midrule
		5&0.5 &0.5 &$22^{\circ}$ & 797.9& 103.1\\ 
		\midrule
		6&0.5 &0.5 &$33^{\circ}$ & 789.2& 101.5 \\ 
		\midrule
		7&0.5 &0.5 &$45^{\circ}$ & 762.5& 101.1  \\ 
		\hline
	\end{tabular}
	\caption{The counting performance on our generated validation set and the real target training set.}
	\label{table:gridsearch}
\end{table*}

==> illustration/backbone.tex <==
\begin{table}[h]
\small
\centering
	\begin{tabular}{c|c|c}
		\toprule
		Input &Layer&Output \\
		\hline
		\midrule
		\multicolumn{3}{c}{$\mathcal{F}$}\\
		\midrule
		3$\times$576$\times$768 & Conv:[k(3,3)-c64-s1-Relu] $\times$ 2 & 64$\times$576$\times$768\\
		\midrule
		64$\times$576$\times$768 & Maxpool:[k(2,2)-s2]  & 64$\times$288$\times$384\\
		\midrule
		64$\times$288$\times$384 & Conv:[k(3,3)-c128-s1-Relu]$\times$ 2  & 128$\times$288$\times$384\\
		\midrule
		128$\times$288$\times$384 & Maxpool:[k(2,2)-s2]  & 128$\times$144$\times$192\\
		\midrule
		128$\times$144$\times$192 & Conv:[k(3,3)-c256-s1-Relu]$\times$ 3  & 256$\times$144$\times$192\\
		\midrule
		256$\times$144$\times$192 & Maxpool:[k(2,2)-s2]  & 256$\times$72$\times$96\\
		\midrule
		256$\times$72$\times$96 & Conv:[k(3,3)-c512-s1-Relu] $\times$ 3 & 512$\times$72$\times$96\\
		\midrule
		\multicolumn{3}{c}{$\mathcal{E}$}\\
		\midrule
		512$\times$72$\times$96 & Conv:[k(3,3)-c128-s1-BN-Relu]  & 128$\times$72$\times$96\\
		\midrule
		128$\times$72$\times$96 & Deconv:[k(2,2)-c128-s2-BN-Relu]  & 128$\times$144$\times$192\\
		\midrule
		128$\times$144$\times$192 & Conv:[k(3,3)-c64-s1-BN-Relu]  & 64$\times$144$\times$192\\
		\midrule
		64$\times$144$\times$192 & Deconv:[k(2,2)-c64-s2-BN-Relu]  & 64$\times$288$\times$384\\
		\midrule
		64$\times$288$\times$384 & Conv:[k(3,3)-c32-s1-BN-Relu]  & 32$\times$288$\times$384\\
		\midrule
		32$\times$288$\times$384 & Deconv:[k(2,2)-c32-s2-BN-Relu]  & 32$\times$576$\times$768\\
		\midrule
		32$\times$576$\times$768 & Conv:[k(3,3)-c1-s1-Relu]  & 32$\times$576$\times$768\\
		\midrule
		\multicolumn{3}{c}{$\mathcal{D}$}\\
		\midrule
		512$\times$72$\times$96 & Conv:[k(3,3)-c512-s1-LeakyReLU]  & 512$\times$72$\times$96\\
		\midrule
		512$\times$72$\times$96 & Conv:[k(3,3)-c256-s1-LeakyReLU]  & 256$\times$72$\times$96\\
		\midrule
		256$\times$72$\times$96 & Conv:[k(3,3)-c2-s1]  & 2$\times$72$\times$96\\
		\midrule
		2$\times$72$\times$96 & Resize  & 2$\times(H/g_{h})\times (W/g_{w})$\\
		\midrule
		\multicolumn{3}{c}{$\mathcal{C}$}\\
		\midrule
		3 & FC:[c16-Relu]  & 16\\
		\midrule
		16 & FC:[c32-Relu]  & 32\\
		\midrule
		32 & FC:[c64-Relu]  & 64\\
		\midrule
		64 & FC:[c1-Relu]  & 1 ($\widetilde p_{k}$)\\
		\midrule
		64 & FC:[c32-Relu]  & 32\\
		\midrule
		32 & FC:[c16-Relu]  & 16\\
		\midrule
		16 & FC:[c3-Relu]  & 3 ($\widetilde d_{k}$)\\
		\hline
	\end{tabular}
	\caption{The network architecture of $\mathcal{F}, \mathcal{E}$, $\mathcal{D}$ and controller $\mathcal{C}$. }
	\label{table:backbone}
\end{table}



==> illustration/grid_search_fig.tex <==
% \begin{figure*}
% \begin{center}

% \begin{minipage}[t]{0.3\linewidth} 
% 	\centering 
% 	\includegraphics[width=1\textwidth]{figs/RGB2Gray.pdf}
% 	\label{figure:grid search gray}
% \end{minipage}
% \hspace{1em}
%   \begin{minipage}[t]{0.3\linewidth} 
%   \centering 
%   \includegraphics[width=1\textwidth]{figs/Scaling.pdf}
%   \label{figure:grid search scale}
%   \end{minipage}
%  \hspace{1em}
%   \begin{minipage}[t]{0.3\linewidth} 
%   \centering 
%   \includegraphics[width=1\textwidth]{figs/PT.pdf}
%   \label{figure:grid search pt}
%   \end{minipage} 
% \end{center}
% \caption{From left to right we search for the three parameters in order. In the left figure, we search for RGB2Gray radio, we find the best radio is 0.5. When searching for the following parameters, we fixed the ratio at 0.5. }
% \label{model}
% \end{figure*}


\begin{figure*}[h]
  \centering
  \includegraphics[scale=0.32]{figs/RGB2Gray.pdf}
  \hspace{1em}
  \includegraphics[scale=0.32]{figs/Scaling.pdf}
  \hspace{1em}
  \includegraphics[scale=0.32]{figs/PT.pdf}
  \caption{\newrevise{From left to right we search for the three parameters in order. $P_G$, scale factor and angle are set to 0., 1.0 and $0^\circ$ by default. In the left figure, we search for $P_G$, and keep scale factor and angle as default, we find the best radio is 0.5. When searching for the following parameters, we fixed the ratio at 0.5. In following search, the parameters searched are fixed as found, and those not searched are kept as default.}
  }
  \label{fig:grid search}
\end{figure*}


==> illustration/small_fig.tex <==
\begin{figure}[t]
	\begin{center}
		% \includegraphics[width=0.95\textwidth]{imgs/module.pdf}
		\includegraphics[width=0.45\textwidth]{figs/small_fig.pdf}
	\end{center}
	\caption{High intraclass diversity samples. Although
	instances belonging to the same class vary greatly  in color, shape and scale, we are required to count them without omission.
% 	\shanshan{The flow is unclear: what is input, loss; maybe we show the baseline and addons from us;}\comment{in progress}
	}
	\label{fig:small_fig}
\end{figure}

==> illustration/srvsst.tex <==
\begin{table}[h]
	\centering
	\begin{tabular}{c|c|c}
		\toprule
		Method & MAE & MSE \\
		\hline
		\midrule
		Cycle-GAN \cite{cyclegan} & 143.3 & 204.3 \\ \midrule
		SE Cycle-GAN \cite{GCC}& 123.4 & 193.4 \\ \midrule
% 		SE Cycle-GAN(JT) \cite{cycleganjt} & 119.6 & 189.1 & 16.4 & 25.8 & 225.9 &385.7 & 370.2 & 512.0 & 24.4\\ \midrule
		SE Cycle-GAN(JT) \cite{cycleganjt} & 119.6 & 189.1 \\  \hline \midrule
		Style Randomization  & 111.6 & 177.5 \\
		\hline
	\end{tabular}
	\caption{\revise{Style Randomization VS Style Transfer.transform(0.5,0.5,22)}}
	\label{table:srvsst}
\end{table}
